Helium Abundance of the Sun: A Spectroscopic Analysis

Determining the He/H ratio in cool stars presents a fundamental astrophysical challenge. While this ratio is established for hot O and B stars, its extrapolation to cool stars remains uncertain due to the absence of helium lines in their observed spectra. We address this knowledge gap by focusing on the Sun as a representative cool star. We conduct spectroscopic analyses of the observed solar photospheric lines by utilizing a combination of MgH molecular lines and neutral Mg atomic lines including yet another combination of CH and C_2 molecular lines with neutral C atomic lines. Our spectroscopic analyses were further exploited by adopting solar model atmospheres constructed for distinct He/H ratios to determine the solar photospheric helium abundance. The helium abundance is determined by enforcing the fact that for an adopted model atmosphere with an appropriate He/H ratio, the derived Mg abundance from the neutral Mg atomic lines and that from the MgH molecular lines must be the same. Ditto holds for the C abundance derived from neutral C atomic lines and that from CH lines of the CH molecular band and C_2 lines from the C_2 Swan band. The estimated He/H ratio for the Sun is discussed based on the one-dimensional local thermodynamic equilibrium (1D LTE) model atmosphere. The helium abundance (He/H = 0.091(+0.019/+0.014)) obtained for the Sun serves as a critical reference point to characterize the He/H ratio of cool stars across the range in their effective temperature. Using this derived He/H ratio, the solar mass fractions are determined to be X_sun=0.7232(+0.0305/-0.0377), Y_sun=0.2633(+0.0384/-0.0311), and Z_sun=0.0135(+0.0006/-0.0007).

==> References.tex <==
@ARTICLE{1929ApJ....70...11R,
       author = {{Russell}, Henry Norris},
        title = "{On the Composition of the Sun's Atmosphere}",
      journal = {\apj},
         year = 1929,
        month = jul,
       volume = {70},
        pages = {11},
          doi = {10.1086/143197},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1929ApJ....70...11R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{RevModPhys.28.53,
  title = {Abundances of the Elements},
  author = {Suess, Hans E. and Urey, Harold C.},
  journal = {Rev. Mod. Phys.},
  volume = {28},
  issue = {1},
  pages = {53--74},
  numpages = {0},
  year = {1956},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.28.53},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.28.53}
}

@article{FOLOMEG1987562,
title = {Vibration-rotation transition probabilities in CH+ and CD+},
journal = {Chemical Physics Letters},
volume = {136},
number = {6},
pages = {562-565},
year = {1987},
issn = {0009-2614},
doi = {https://doi.org/10.1016/0009-2614(87)80518-3},
url = {https://www.sciencedirect.com/science/article/pii/0009261487805183},
author = {B. Folomeg and P. Rosmus and H.-J. Werner},
abstract = {Vibrational dipole matrix elements and radiative transition probabilities have been evaluated from electric dipole moment functions for the X1Σ+ states of CH+ and CD+, which were calculated from highly correlated electronic wavefunctions. The dipole moments in ν = 0 amount to 1.679 D (CH+) and 1.313 D (CD+), respectively. In comparison to other molecular ions the infrared transition probabilities are found to be rather small. For instance, the Einstein coefficient of spontaneous emission A10 amounts to 1.63 s−1 (CH+) and 0.19 s−1 (CD+). Dipole moment functions of the neutral CH species in the X2Π and a4 Σ− states have also been calculated and are compared with previous theoretical functions.}
}

@ARTICLE{1960ApJS....5....1G,
       author = {{Goldberg}, Leo and {Muller}, Edith A. and {Aller}, Lawrence H.},
        title = "{The Abundances of the Elements in the Solar Atmosphere.}",
      journal = {\apjs},
         year = 1960,
        month = nov,
       volume = {5},
        pages = {1},
          doi = {10.1086/190053},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1960ApJS....5....1G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1968MNRAS.138..143L,
       author = {{Lambert}, D.~L.},
        title = "{The abundances of the elements in the solar photosphere-I, Carbon, nitrogen and oxygen}",
      journal = {\mnras},
         year = 1968,
        month = jan,
       volume = {138},
        pages = {143},
          doi = {10.1093/mnras/138.2.143},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1968MNRAS.138..143L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1967Natur.215...43L,
       author = {{Lambert}, D.~L.},
        title = "{Abundance of Helium in the Sun}",
      journal = {\nat},
         year = 1967,
        month = jul,
       volume = {215},
       number = {5096},
        pages = {43-44},
          doi = {10.1038/215043a0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1967Natur.215...43L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1973RvGSP..11..115H,
       author = {{Hirshberg}, J.},
        title = "{Helium Abundance of the Sun}",
      journal = {Reviews of Geophysics and Space Physics},
         year = 1973,
        month = feb,
       volume = {11},
        pages = {115},
          doi = {10.1029/RG011i001p00115},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1973RvGSP..11..115H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{2021LNP...978.....R,
       author = {{Reames}, Donald V.},
        title = "{Solar Energetic Particles. A Modern Primer on Understanding Sources, Acceleration and Propagation}",
         year = 2021,
       volume = {978},
          doi = {10.1007/978-3-030-66402-2},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021LNP...978.....R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2004ApJ...606L..85B,
       author = {{Basu}, Sarbani and {Antia}, H.~M.},
        title = "{Constraining Solar Abundances Using Helioseismology}",
      journal = {\apjl},
     keywords = {Sun: Abundances, Sun: Interior, Sun: Oscillations, Astrophysics},
         year = 2004,
        month = may,
       volume = {606},
       number = {1},
        pages = {L85-L88},
          doi = {10.1086/421110},
archivePrefix = {arXiv},
       eprint = {astro-ph/0403485},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004ApJ...606L..85B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008PhR...457..217B,
       author = {{Basu}, Sarbani and {Antia}, H.~M.},
        title = "{Helioseismology and solar abundances}",
      journal = {\physrep},
     keywords = {Astrophysics},
         year = 2008,
        month = mar,
       volume = {457},
       number = {5-6},
        pages = {217-283},
          doi = {10.1016/j.physrep.2007.12.002},
archivePrefix = {arXiv},
       eprint = {0711.4590},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008PhR...457..217B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014SoPh..289..977R,
       author = {{Reames}, Donald V.},
        title = "{Element Abundances in Solar Energetic Particles and the Solar Corona}",
      journal = {\solphys},
     keywords = {Solar energetic particles, Shock waves, Coronal mass ejections, Solar system abundances, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = mar,
       volume = {289},
       number = {3},
        pages = {977-993},
          doi = {10.1007/s11207-013-0350-4},
archivePrefix = {arXiv},
       eprint = {1306.2246},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014SoPh..289..977R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014MNRAS.441.3296V,
       author = {{Vorontsov}, S.~V. and {Baturin}, V.~A. and {Ayukov}, S.~V. and {Gryaznov}, V.~K.},
        title = "{Helioseismic measurements in the solar envelope using group velocities of surface waves}",
      journal = {\mnras},
     keywords = {equation of state, waves, Sun: abundances, Sun: helioseismology, Sun: oscillations, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = jul,
       volume = {441},
       number = {4},
        pages = {3296-3305},
          doi = {10.1093/mnras/stu813},
archivePrefix = {arXiv},
       eprint = {1402.0204},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.441.3296V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1989GeCoA..53..197A,
       author = {{Anders}, E. and {Grevesse}, N.},
        title = "{Abundances of the elements: Meteoritic and solar}",
      journal = {\gca},
     keywords = {Abundance, Chemical Analysis, Chondrites, Meteoritic Composition, Photosphere, Solar Corona, Energetic Particles, Isotopes, Solar Wind, METEORITES, ABUNDANCE, SAMPLES, METEORITE, CI CHONDRITES, SUN, CORONA, PHOTOSPHERE, REVIEW, ELEMENTS, FRACTIONATION, SOLAR SYSTEM, NUCLIDES, SOLAR WIND, CHARGED PARTICLES, RARE GASES, REFRACTORY ELEMENTS, COMETS, SIDEROPHILES, VOLATILES, NUCLEOSYNTHESIS, HALLEY, COMPARISONS},
         year = 1989,
        month = jan,
       volume = {53},
       number = {1},
        pages = {197-214},
          doi = {10.1016/0016-7037(89)90286-X},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1989GeCoA..53..197A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1998SSRv...85..161G,
       author = {{Grevesse}, N. and {Sauval}, A.~J.},
        title = "{Standard Solar Composition}",
      journal = {\ssr},
     keywords = {Sun: abundances, Meteorites: abundances, Solar spectroscopy},
         year = 1998,
        month = may,
       volume = {85},
        pages = {161-174},
          doi = {10.1023/A:1005161325181},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998SSRv...85..161G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ApJ...591.1220L,
       author = {{Lodders}, Katharina},
        title = "{Solar System Abundances and Condensation Temperatures of the Elements}",
      journal = {\apj},
     keywords = {Astrochemistry, Meteors, Meteoroids, Solar System: Formation- Sun: Abundances, Sun: Photosphere},
         year = 2003,
        month = jul,
       volume = {591},
       number = {2},
        pages = {1220-1247},
          doi = {10.1086/375492},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...591.1220L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2005ASPC..336...25A,
       author = {{Asplund}, M. and {Grevesse}, N. and {Sauval}, A.~J.},
        title = "{The Solar Chemical Composition}",
    booktitle = {Cosmic Abundances as Records of Stellar Evolution and Nucleosynthesis},
         year = 2005,
       editor = {{Barnes}, Thomas G., III and {Bash}, Frank N.},
       series = {Astronomical Society of the Pacific Conference Series},
       volume = {336},
        month = sep,
        pages = {25},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ASPC..336...25A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2009ARA&A..47..481A,
       author = {{Asplund}, Martin and {Grevesse}, Nicolas and {Sauval}, A. Jacques and {Scott}, Pat},
        title = "{The Chemical Composition of the Sun}",
      journal = {\araa},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2009,
        month = sep,
       volume = {47},
       number = {1},
        pages = {481-522},
          doi = {10.1146/annurev.astro.46.060407.145222},
archivePrefix = {arXiv},
       eprint = {0909.0948},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ARA&A..47..481A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020JApA...41...41A,
       author = {{Allende Prieto}, Carlos},
        title = "{Chemical composition of the solar surface}",
      journal = {Journal of Astrophysics and Astronomy},
     keywords = {The Sun, chemical composition, stellar atmospheres, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = dec,
       volume = {41},
       number = {1},
          eid = {41},
        pages = {41},
          doi = {10.1007/s12036-020-09666-3},
archivePrefix = {arXiv},
       eprint = {2106.10750},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020JApA...41...41A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019arXiv191200844L,
       author = {{Lodders}, Katharina},
        title = "{Solar Elemental Abundances}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2019,
        month = dec,
          eid = {arXiv:1912.00844},
        pages = {arXiv:1912.00844},
          doi = {10.48550/arXiv.1912.00844},
archivePrefix = {arXiv},
       eprint = {1912.00844},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv191200844L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1969SoPh....8..435O,
       author = {{Ogilvie}, K.~W. and {Wilkerson}, T.~D.},
        title = "{Helium Abundance in the Solar Wind}",
      journal = {\solphys},
     keywords = {Hydrogen, Magnetic Field, Helium, Recent Work, Solar Wind},
         year = 1969,
        month = aug,
       volume = {8},
       number = {2},
        pages = {435-449},
          doi = {10.1007/BF00155391},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1969SoPh....8..435O},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1984sfat.book.....K,
       author = {{Kurucz}, Robert L. and {Furenlid}, Ingemar and {Brault}, James and {Testerman}, Larry},
        title = "{Solar flux atlas from 296 to 1300 nm}",
         year = 1984,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1984sfat.book.....K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1998A&AS..131..431A,
       author = {{Allende Prieto}, C. and {Garcia Lopez}, R.~J.},
        title = "{A catalogue of accurate wavelengths in the optical spectrum of the Sun}",
      journal = {\aaps},
     keywords = {LINE: IDENTIFICATION, TECHNIQUES: SPECTROSCOPIC, CATALOGS, SUN: PHOTOSPHERE, Astrophysics},
         year = 1998,
        month = sep,
       volume = {131},
        pages = {431-433},
          doi = {10.1051/aas:1998280},
archivePrefix = {arXiv},
       eprint = {astro-ph/9803262},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998A&AS..131..431A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{2000vnia.book.....H,
       author = {{Hinkle}, Kenneth and {Wallace}, Lloyd and {Valenti}, Jeff and {Harmer}, Dianne},
        title = "{Visible and Near Infrared Atlas of the Arcturus Spectrum 3727-9300 A}",
         year = 2000,
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000vnia.book.....H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INCOLLECTION{2014dapb.book...39K,
       author = {{Kurucz}, Robert L.},
        title = "{Model Atmosphere Codes: ATLAS12 and ATLAS9}",
    booktitle = {Determination of Atmospheric Parameters of B},
         year = 2014,
        pages = {39-51},
          doi = {10.1007/978-3-319-06956-2_4},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014dapb.book...39K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2020ApJ...897...32H,
       author = {{Hema}, B.~P. and {Pandey}, Gajendra and {Kurucz}, R.~L. and {Allende Prieto}, C.},
        title = "{Helium Enhancement in the Metal-rich Red Giants of {\ensuremath{\omega}} Centauri}",
      journal = {\apj},
     keywords = {Globular star clusters, Chemical abundances, Red giant stars, Hydrogen deficient stars, Chemically peculiar stars, Stellar evolutionary tracks, 769, 224, 1600, 656, 226, 1372, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jul,
       volume = {897},
       number = {1},
          eid = {32},
        pages = {32},
          doi = {10.3847/1538-4357/ab93bd},
archivePrefix = {arXiv},
       eprint = {2005.06807},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020ApJ...897...32H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{2012ascl.soft02009S,
       author = {{Sneden}, Chris and {Bean}, Jacob and {Ivans}, Inese and {Lucatello}, Sara and {Sobeck}, Jennifer},
        title = "{MOOG: LTE line analysis and spectrum synthesis}",
     keywords = {Software, NASA},
 howpublished = {Astrophysics Source Code Library, record ascl:1202.009},
         year = 2012,
        month = feb,
          eid = {ascl:1202.009},
        pages = {ascl:1202.009},
archivePrefix = {ascl},
       eprint = {1202.009},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ascl.soft02009S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...539A.143N,
       author = {{Nieva}, M. -F. and {Przybilla}, N.},
        title = "{Present-day cosmic abundances. A comprehensive study of nearby early B-type stars and implications for stellar and Galactic evolution and interstellar dust models}",
      journal = {\aap},
     keywords = {stars: abundances, stars: early-type, stars: fundamental parameters, stars: evolution, ISM: abundances, Galaxy: evolution, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Cosmology and Extragalactic Astrophysics, Astrophysics - Galaxy Astrophysics},
         year = 2012,
        month = mar,
       volume = {539},
          eid = {A143},
        pages = {A143},
          doi = {10.1051/0004-6361/201118158},
archivePrefix = {arXiv},
       eprint = {1203.5787},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...539A.143N},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015LRSP...12....2L,
       author = {{Laming}, J. Martin},
        title = "{The FIP and Inverse FIP Effects in Solar and Stellar Coronae}",
      journal = {Living Reviews in Solar Physics},
     keywords = {Stellar coronae, Waves, Turbulence, Corona, Abundances, Chromosphere, Stars: coronae, Sun: abundances, Sun: chromosphere, Sun: corona, Astrophysics - Solar and Stellar Astrophysics},
         year = 2015,
        month = sep,
       volume = {12},
       number = {1},
          eid = {2},
        pages = {2},
          doi = {10.1007/lrsp-2015-2},
archivePrefix = {arXiv},
       eprint = {1504.08325},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015LRSP...12....2L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011SoPh..268..255C,
       author = {{Caffau}, E. and {Ludwig}, H. -G. and {Steffen}, M. and {Freytag}, B. and {Bonifacio}, P.},
        title = "{Solar Chemical Abundances Determined with a CO5BOLD 3D Model Atmosphere}",
      journal = {\solphys},
     keywords = {Sun: abundances, Sun: photosphere, Line: formation, Hydrodynamics, Convection, Radiative transfer, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = feb,
       volume = {268},
       number = {2},
        pages = {255-269},
          doi = {10.1007/s11207-010-9541-4},
archivePrefix = {arXiv},
       eprint = {1003.1190},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011SoPh..268..255C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@online{kurucz93,
  author = {{Kurucz}, R.~L.},
  title = {Robert L. Kurucz},
  year = 1993,
  url = {http://kurucz.harvard.edu/}
}

@ARTICLE{2017A&A...598A.102P,
       author = {{Pehlivan Rhodin}, A. and {Hartman}, H. and {Nilsson}, H. and {J{\"o}nsson}, P.},
        title = "{Experimental and theoretical oscillator strengths of Mg I for accurate abundance analysis}",
      journal = {\aap},
     keywords = {atomic data, methods: laboratory: atomic, techniques: spectroscopic, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2017,
        month = feb,
       volume = {598},
          eid = {A102},
        pages = {A102},
          doi = {10.1051/0004-6361/201629849},
archivePrefix = {arXiv},
       eprint = {1611.07000},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...598A.102P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2008A&A...486..951G,
       author = {{Gustafsson}, B. and {Edvardsson}, B. and {Eriksson}, K. and {J{\o}rgensen}, U.~G. and {Nordlund}, {\r{A}}. and {Plez}, B.},
        title = "{A grid of MARCS model atmospheres for late-type stars. I. Methods and general properties}",
      journal = {\aap},
     keywords = {stars: atmospheres, Sun: abundances, stars: fundamental parameters, stars: general, stars: late-type, stars: supergiants, Astrophysics},
         year = 2008,
        month = aug,
       volume = {486},
       number = {3},
        pages = {951-970},
          doi = {10.1051/0004-6361:200809724},
archivePrefix = {arXiv},
       eprint = {0805.0554},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...486..951G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1974SoPh...39...19H,
       author = {{Holweger}, H. and {Mueller}, E.~A.},
        title = "{The Photospheric Barium Spectrum: Solar Abundance and Collision Broadening of Ba II Lines by Hydrogen}",
      journal = {\solphys},
     keywords = {Atmospheric Models, Atomic Collisions, Barium, Photosphere, Solar Spectra, Spectral Line Width, Abundance, Astronomical Models, Hydrogen Atoms, Line Spectra, Metal Ions, Metastable State, Solar Atmosphere, Solar Physics, Hydrogen Atom, Barium, Resonance Line, Solar Spectrum, Equivalent Width},
         year = 1974,
        month = nov,
       volume = {39},
       number = {1},
        pages = {19-30},
          doi = {10.1007/BF00154968},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1974SoPh...39...19H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1967ZA.....65..365H,
       author = {{Holweger}, H.},
        title = "{Ein empirisches Modell der Sonnenatmosph{\"a}re mit lokalem thermodynamischem Gleichgewicht}",
      journal = {\zap},
         year = 1967,
        month = jan,
       volume = {65},
        pages = {365},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1967ZA.....65..365H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2021A&A...653A.141A,
       author = {{Asplund}, M. and {Amarsi}, A.~M. and {Grevesse}, N.},
        title = "{The chemical make-up of the Sun: A 2020 vision}",
      journal = {\aap},
     keywords = {Sun: abundances, Sun: photosphere, Sun: atmosphere, line: formation, meteorites, meteors, meteoroids, Sun: helioseismology, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Earth and Planetary Astrophysics},
         year = 2021,
        month = sep,
       volume = {653},
          eid = {A141},
        pages = {A141},
          doi = {10.1051/0004-6361/202140445},
archivePrefix = {arXiv},
       eprint = {2105.01661},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...653A.141A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2000A&A...359..743A,
       author = {{Asplund}, M. and {Nordlund}, {\r{A}}. and {Trampedach}, R. and {Stein}, R.~F.},
        title = "{Line formation in solar granulation. II. The photospheric Fe abundance}",
      journal = {\aap},
     keywords = {CONVECTION, HYDRODYNAMICS, LINE: FORMATION, SUN: ABUNDANCES, SUN: GRANULATION, SUN: PHOTOSPHERE, Astrophysics},
         year = 2000,
        month = jul,
       volume = {359},
        pages = {743-754},
          doi = {10.48550/arXiv.astro-ph/0005321},
archivePrefix = {arXiv},
       eprint = {astro-ph/0005321},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2000A&A...359..743A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1979ApJ...231..637K,
       author = {{Kirby}, K. and {Saxon}, R.~P. and {Liu}, B.},
        title = "{Oscillator Strengths and Photodissociation Cross Sections in the X-->A and X-->B' Band Systems in MgH}",
      journal = {\apj},
         year = 1979,
        month = jul,
       volume = {231},
        pages = {637-644},
          doi = {10.1086/157226},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1979ApJ...231..637K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003ApJ...582.1059W,
       author = {{Weck}, P.~F. and {Schweitzer}, A. and {Stancil}, P.~C. and {Hauschildt}, P.~H. and {Kirby}, K.},
        title = "{The Molecular Line Opacity of MgH in Cool Stellar Atmospheres}",
      journal = {\apj},
     keywords = {Molecular Data, Stars: Atmospheres, Stars: Late-Type, Astrophysics},
         year = 2003,
        month = jan,
       volume = {582},
       number = {2},
        pages = {1059-1065},
          doi = {10.1086/344722},
archivePrefix = {arXiv},
       eprint = {astro-ph/0206219},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...582.1059W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@book{gray_2021, place={Cambridge}, edition={4}, title={The Observation and Analysis of Stellar Photospheres}, DOI={10.1017/9781009082136}, publisher={Cambridge University Press}, author={Gray, David F.}, year={2021}}

@book{banwell1994fundamentals,
  title={Fundamentals of Molecular Spectroscopy},
  author={Banwell, C.N. and McCash, E.M.},
  isbn={9780077079765},
  lccn={94000869},
  url={https://books.google.co.in/books?id=CJwgnwEACAAJ},
  year={1994},
  publisher={McGraw-Hill}
}

@ARTICLE{1971MNRAS.154..265L,
       author = {{Lambert}, D.~L. and {Mallia}, E.~A. and {Petford}, A.~D.},
        title = "{Magnesium hydride in theSun}",
      journal = {\mnras},
         year = 1971,
        month = jan,
       volume = {154},
        pages = {265},
          doi = {10.1093/mnras/154.3.265},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1971MNRAS.154..265L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1973A&A....27...29G,
       author = {{Grevesse}, N. and {Sauval}, A.~J.},
        title = "{A Study of Molecular Lines in the Solar Photospheric Spectrum}",
      journal = {\aap},
         year = 1973,
        month = aug,
       volume = {27},
        pages = {29},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1973A&A....27...29G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PROCEEDINGS{1977egsp.conf.....T,
        title = "{Evolution of galaxies and stellar populations}",
     keywords = {GALAXIES, STELLAR POPULATIONS, DYNAMICAL EVOLUTION, CHEMICAL EVOLUTION, CONFERENCES, GALAXIES: EVOLUTION: CONGRESSES, STARS: EVOLUTION: CONGRESSES, STARS: POPULATIONS},
    booktitle = {Evolution of Galaxies and Stellar Populations},
         year = 1977,
        month = jan,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1977egsp.conf.....T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014ApJ...792L..28H,
       author = {{Hema}, B.~P. and {Pandey}, Gajendra},
        title = "{Discovery of Relatively Hydrogen-poor Giants in the Galactic Globular Cluster {\ensuremath{\omega}} Centauri}",
      journal = {\apjl},
     keywords = {globular clusters: general, globular clusters: individual: Omega Centauri, stars: chemically peculiar, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = sep,
       volume = {792},
       number = {2},
          eid = {L28},
        pages = {L28},
          doi = {10.1088/2041-8205/792/2/L28},
archivePrefix = {arXiv},
       eprint = {1408.1205},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...792L..28H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018ApJ...864..121H,
       author = {{Hema}, B.~P. and {Pandey}, Gajendra and {Srianand}, R.},
        title = "{High-resolution Spectroscopy of the Relatively Hydrogen-poor Metal-rich Giants in the Globular Cluster {\ensuremath{\omega}} Centauri}",
      journal = {\apj},
     keywords = {globular clusters: individual: Omega Centauri, stars: abundances, stars: chemically peculiar, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2018,
        month = sep,
       volume = {864},
       number = {2},
          eid = {121},
        pages = {121},
          doi = {10.3847/1538-4357/aad696},
archivePrefix = {arXiv},
       eprint = {1807.10813},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...864..121H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2013MNRAS.432.2043G,
       author = {{GharibNezhad}, Ehsan and {Shayesteh}, Alireza and {Bernath}, Peter F.},
        title = "{Einstein A coefficients for rovibronic lines of the A $^{2}$ {\ensuremath{\Pi}} {\textrightarrow} X $^{2}${\ensuremath{\Sigma}}$^{+}$ and B' $^{2}${\ensuremath{\Sigma}}$^{+}${\textrightarrow} X $^{2}$ {\ensuremath{\Sigma}}$^{+}$ transitions of MgH}",
      journal = {\mnras},
     keywords = {molecular data, stars: late-type, subdwarfs},
         year = 2013,
        month = jul,
       volume = {432},
       number = {3},
        pages = {2043-2047},
          doi = {10.1093/mnras/stt510},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.432.2043G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{alma991043245695503276,
abstract = {1. Introduction. 1.1. Waves, Particles, and Units. 1.2. The Electromagnetic Spectrum. 1.3. Interaction of Radiation with Matter. 1.3a. Blackbody Radiation. 1.3b. Einstein A and B Coefficients. 1.3c. Absorption and Emission of Radiation. 1.3d. Beer's Law. 1.3e. Lineshape Functions. 1.3f. Natural Lifetime Broadening. 1.3g. Pressure Broadening. 1.3h. Doppler Broadening. 1.3i. Transit-Time Broadening. 1.3j. Power Broadening. 2. Molecular Symmetry. 2.1. Symmetry Operations. 2.1a. Operator Algebra. 2.1b. Symmetry Operator Algebra. 2.2. Groups. 2.2a. Point Groups. 2.2b. Classes. 2.2c. Subgroups. 2.3.},
author = {Bernath, Peter F.},
address = {New York},
booktitle = {Spectra of atoms and molecules},
edition = {2nd ed.},
isbn = {1-280-70444-6},
publisher = {Oxford University Press},
title = {Spectra of atoms and molecules [electronic resource] / Peter F. Bernath.},
year = {2005},
language = {eng},
lccn = {2004062020},
keywords = {Atomic spectroscopy -- Textbooks},
}

@ARTICLE{2014ApJS..211....5R,
       author = {{Ram}, Ram S. and {Brooke}, James S.~A. and {Bernath}, Peter F. and {Sneden}, Christopher and {Lucatello}, Sara},
        title = "{Improved Line Data for the Swan System $^{12}$C$^{13}$C Isotopologue}",
      journal = {\apjs},
     keywords = {line: identification, molecular data, stars: abundances, stars: carbon, stars: individual: Arcturus HE 0212-0557},
         year = 2014,
        month = mar,
       volume = {211},
       number = {1},
          eid = {5},
        pages = {5},
          doi = {10.1088/0067-0049/211/1/5},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJS..211....5R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2014A&A...571A..47M,
       author = {{Masseron}, T. and {Plez}, B. and {Van Eck}, S. and {Colin}, R. and {Daoutidis}, I. and {Godefroid}, M. and {Coheur}, P. -F. and {Bernath}, P. and {Jorissen}, A. and {Christlieb}, N.},
        title = "{CH in stellar atmospheres: an extensive linelist}",
      journal = {\aap},
     keywords = {molecular data, techniques: spectroscopic, stars: carbon, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = nov,
       volume = {571},
          eid = {A47},
        pages = {A47},
          doi = {10.1051/0004-6361/201423956},
archivePrefix = {arXiv},
       eprint = {1410.4005},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...571A..47M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1974ApJS...27....1W,
       author = {{Whiting}, Ellis E. and {Nicholls}, Ralph W.},
        title = "{Reinvestigation of Rotational-Line Intensity Factors in Diatomic Spectra}",
      journal = {\apjs},
         year = 1974,
        month = jan,
       volume = {27},
        pages = {1},
          doi = {10.1086/190286},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1974ApJS...27....1W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{10.1063/1.1675084,
    author = {Henneker, W. H. and Popkie, H. E.},
    title = "{Theoretical Electronic Transition Probabilities in Diatomic Molecules. I. Hydrides}",
    journal = {The Journal of Chemical Physics},
    volume = {54},
    number = {4},
    pages = {1763-1778},
    year = {2003},
    month = {09},
    abstract = "{Hartree–Fock (HF) electronic transition moments calculated in both the position and momentum representations are presented as a function of the internuclear separation R for the BeH, MgH, OH, and SH (A–X) systems. The vibrational averages of these quantities are obtained and the results are used to calculate some absorption band oscillator strengths. For the OH (A–X) system several independent experimental determinations of the 0–0 band oscillator strength have been reported in the literature. Our theoretical value of 20.6 × 10−4 differs from experiment by a factor of 2.5. Active electron and virtual orbital approximations to the HF transition moment integrals are given. Consideration of the united and separated atom limits and the region of the equilibrium internuclear separation for the states involved leads to an abbreviated discussion of the effect of correlation on the HF transition moments. HF transition moment calculations at a single value of R are also reported for the BH+, AlH+, HF+, and HCl+ (A–X) systems.}",
    issn = {0021-9606},
    doi = {10.1063/1.1675084},
    url = {https://doi.org/10.1063/1.1675084},
    eprint = {https://pubs.aip.org/aip/jcp/article-pdf/54/4/1763/11319778/1763\_1\_online.pdf},
}

@article{10.1063/1.1673619,
    author = {Chan, Arthur C. H. and Davidson, Ernest R.},
    title = "{Theoretical Study of the MgH Molecule}",
    journal = {The Journal of Chemical Physics},
    volume = {52},
    number = {8},
    pages = {4108-4121},
    year = {2003},
    month = {09},
    abstract = "{Within the Born–Oppenheimer framework, extended configuration‐interaction calculations, involving the use of natural orbitals, are carried out to study the ground‐state energy, wavefunction, and selected molecular properties at the experimental equilibrium internuclear separation of the MgH molecule. Electronic population analysis of the elaborate molecular wavefunctions is done to investigate the nature of the chemical bond involved. More limited configuration‐interaction calculations are also carried out to study the low‐lying excited states of the MgH molecule. Potential‐energy curves are plotted, and transition probabilities are also considered. An estimated dissociation energy of 2.0 ± 0.2 eV has been deduced for the MgH molecule. A dipole moment of − 0.595 a.u. (− 1.511 D) was also obtained. The various results obtained confirmed the intuitive belief that the BeH and the MgH molecules are cogeners. Careful analysis of the accurate molecular wavefunctions reveals that the promotion of an s electron to the corresponding p orbital in bond formation is characteristic of the BeH and the MgH molecules. The calculated transition energy (A 2Π → X 2Σ+) for the MgH molecule was within 5\\% of the experimental value.}",
    issn = {0021-9606},
    doi = {10.1063/1.1673619},
    url = {https://doi.org/10.1063/1.1673619},
    eprint = {https://pubs.aip.org/aip/jcp/article-pdf/52/8/4108/11275198/4108\_1\_online.pdf},
}

@article{10.1063/1.1674728,
    author = {Popkie, H. E.},
    title = "{Theoretical Electronic Transition Probabilities in Diatomic Molecules. III BeH and MgH (A 2Π–X 2Σ+) Systems}",
    journal = {The Journal of Chemical Physics},
    volume = {54},
    number = {11},
    pages = {4597-4605},
    year = {2003},
    month = {09},
    abstract = "{Electronic dipole‐momentum and dipole‐length transition moment curves obtained from the multiconfiguration (MC) wavefunctions of Chan and Davidson are presented for the BeH and MgH (A 2Π–X 2Σ+) systems. They are used to discuss the correlation correction to the Hartree–Fock (HF) curves previously reported. The MC transition moments and vibrational wavefunctions derived from both the theoretical MC and “experimental” RKR potential‐energy curves for the A 2Π and X 2Σ+ states are used to calculate band oscillator strengths. A table of band wavelengths and semitheoretical transition probabilities is presented for each system and the predicted band spectrum is briefly discussed.}",
    issn = {0021-9606},
    doi = {10.1063/1.1674728},
    url = {https://doi.org/10.1063/1.1674728},
    eprint = {https://pubs.aip.org/aip/jcp/article-pdf/54/11/4597/10990949/4597\_1\_online.pdf},
}

@phdthesis{hdstars,
    title        = {Investigations of Hydrogen Deficient Stars and Related Objects},
    author       = {{Pandey}, G.},
    year         = 1999,
    month        = {September},
    school       = {Indian Institute of Astrophysics},
    address      = {Bengaluru},
    note         = {Available at \url{http://prints.iiap.res.in/handle/2248/97}},
    type         = {PhD thesis}
}

@ARTICLE{2015A&A...573A..25S,
       author = {{Scott}, Pat and {Grevesse}, Nicolas and {Asplund}, Martin and {Sauval}, A. Jacques and {Lind}, Karin and {Takeda}, Yoichi and {Collet}, Remo and {Trampedach}, Regner and {Hayek}, Wolfgang},
        title = "{The elemental composition of the Sun. I. The intermediate mass elements Na to Ca}",
      journal = {\aap},
     keywords = {Sun: abundances, Sun: photosphere, Sun: granulation, line:, formation, line: profiles, convection, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Earth and Planetary Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = jan,
       volume = {573},
          eid = {A25},
        pages = {A25},
          doi = {10.1051/0004-6361/201424109},
archivePrefix = {arXiv},
       eprint = {1405.0279},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...573A..25S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013ApJS..207...26H,
       author = {{Hinkle}, Kenneth H. and {Wallace}, Lloyd and {Ram}, Ram S. and {Bernath}, Peter F. and {Sneden}, Christopher and {Lucatello}, Sara},
        title = "{The Magnesium Isotopologues of MgH in the A $^{2}${\ensuremath{\Pi}}-X $^{2}${\ensuremath{\Sigma}}$^{+}$ System}",
      journal = {\apjs},
     keywords = {molecular data, stars: abundances, stars: late-type, sunspots},
         year = 2013,
        month = aug,
       volume = {207},
       number = {2},
          eid = {26},
        pages = {26},
          doi = {10.1088/0067-0049/207/2/26},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJS..207...26H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1991A&A...242..488G,
       author = {{Grevesse}, N. and {Lambert}, D.~L. and {Sauval}, A.~J. and {van Dishoeck}, E.~F. and {Farmer}, C.~B. and {Norton}, R.~H.},
        title = "{Vibration-rotation bands of CH in the solar infrared spectrum and the solar carbon abundance}",
      journal = {\aap},
     keywords = {Carbon, Hydrocarbons, Infrared Spectra, Rotational Spectra, Solar Spectra, Vibrational Spectra, Abundance, Electron Transitions, High Resolution, Molecular Excitation, Solar Spectrometers, Solar Physics},
         year = 1991,
        month = feb,
       volume = {242},
       number = {2},
        pages = {488-495},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991A&A...242..488G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012ApJ...747..102H,
       author = {{Hema}, B.~P. and {Pandey}, Gajendra and {Lambert}, David L.},
        title = "{The Galactic R Coronae Borealis Stars: The C$_{2}$ Swan Bands, the Carbon Problem, and the $^{12}$C/$^{13}$C Ratio}",
      journal = {\apj},
     keywords = {stars: abundances, stars: chemically peculiar, stars: evolution, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = mar,
       volume = {747},
       number = {2},
          eid = {102},
        pages = {102},
          doi = {10.1088/0004-637X/747/2/102},
archivePrefix = {arXiv},
       eprint = {1201.1357},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...747..102H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{10.1063/1.2806988,
    author = {Schmidt, Timothy W. and Bacskay, George B.},
    title = "{Oscillator strengths of the Mulliken, Swan, Ballik-Ramsay, Phillips, and dΠg3←cΣu+3 systems of C2 calculated by MRCI methods utilizing a biorthogonal transformation of CASSCF orbitals}",
    journal = {The Journal of Chemical Physics},
    volume = {127},
    number = {23},
    pages = {234310},
    year = {2007},
    month = {12},
    abstract = "{Ab initio oscillator strengths and lifetimes for the DΣu+1←XΣg+1 Mulliken system of C2 are reported. The calculations were carried out at the MRCI level of theory with Davidson’s correction using aug-cc-pV6Z basis sets and include core and core-valence correlation as well as relativistic corrections, computed with aug-cc-pCVQZ and cc-pVQZ bases, respectively. The MRCI calculations of transition moments utilize a biorthogonal transformation of the CASSCF orbitals. This approach was also employed to recompute the transition moments of the Swan, Ballik-Ramsay, Phillips, and dΠg3←cΣu+3 systems of C2, which were the subject of our previous study [D. L. Kokkin et al., J. Chem. Phys. 126, 084302 (2007)], resulting in an improved set of oscillator strengths for the latter systems as well. The oscillator strength of the Mulliken origin band, f00DA, was calculated to be 0.0535, in excellent agreement with the accepted astronomical value of 0.054.}",
    issn = {0021-9606},
    doi = {10.1063/1.2806988},
    url = {https://doi.org/10.1063/1.2806988},
    eprint = {https://pubs.aip.org/aip/jcp/article-pdf/doi/10.1063/1.2806988/15407815/234310\_1\_online.pdf},
}


@ARTICLE{2013JQSRT.124...11B,
       author = {{Brooke}, James S.~A. and {Bernath}, Peter F. and {Schmidt}, Timothy W. and {Bacskay}, George B.},
        title = "{Line strengths and updated molecular constants for the C$_{2}$ Swan system}",
      journal = {\jqsrt},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Physics - Chemical Physics},
         year = 2013,
        month = jul,
       volume = {124},
        pages = {11-20},
          doi = {10.1016/j.jqsrt.2013.02.025},
archivePrefix = {arXiv},
       eprint = {1212.2102},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013JQSRT.124...11B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2019A&A...624A.111A,
       author = {{Amarsi}, A.~M. and {Barklem}, P.~S. and {Collet}, R. and {Grevesse}, N. and {Asplund}, M.},
        title = "{3D non-LTE line formation of neutral carbon in the Sun}",
      journal = {\aap},
     keywords = {atomic data, radiative transfer, line: formation, Sun: abundances, Sun: photosphere, Astrophysics - Solar and Stellar Astrophysics},
         year = 2019,
        month = apr,
       volume = {624},
          eid = {A111},
        pages = {A111},
          doi = {10.1051/0004-6361/201833603},
archivePrefix = {arXiv},
       eprint = {1903.08838},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...624A.111A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005A&A...431..693A,
       author = {{Asplund}, M. and {Grevesse}, N. and {Sauval}, A.~J. and {Allende Prieto}, C. and {Blomme}, R.},
        title = "{Line formation in solar granulation. VI. [C I], C I, CH and C$_{2}$ lines and the photospheric C abundance}",
      journal = {\aap},
     keywords = {convection, line: formation, Sun: abundances, Sun: granulation, Sun: photosphere, stars: atmospheres, Astrophysics},
         year = 2005,
        month = feb,
       volume = {431},
        pages = {693-705},
          doi = {10.1051/0004-6361:20041951},
archivePrefix = {arXiv},
       eprint = {astro-ph/0410681},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005A&A...431..693A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012MNRAS.422..542P,
       author = {{Pavlenko}, Ya. V. and {Jenkins}, J.~S. and {Jones}, H.~R.~A. and {Ivanyuk}, O. and {Pinfield}, D.~J.},
        title = "{Effective temperatures, rotational velocities, microturbulent velocities and abundances in the atmospheres of the Sun, HD 1835 and HD 10700}",
      journal = {\mnras},
     keywords = {stars: abundances, stars: evolution, stars: fundamental parameters, stars: late-type, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = may,
       volume = {422},
       number = {1},
        pages = {542-552},
          doi = {10.1111/j.1365-2966.2012.20629.x},
archivePrefix = {arXiv},
       eprint = {1201.5099},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012MNRAS.422..542P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2022A&A...668A...9H,
       author = {{Hong}, Jie and {Qiu}, Ye and {Hao}, Qi and {Xu}, Zhi and {Li}, Chuan and {Ding}, Mingde and {Fang}, Cheng},
        title = "{Statistical analysis of the Si I 6560.58 {\r{A}} line observed by CHASE}",
      journal = {\aap},
     keywords = {line: formation, line: profiles, Sun: photosphere, turbulence, Astrophysics - Solar and Stellar Astrophysics},
         year = 2022,
        month = dec,
       volume = {668},
          eid = {A9},
        pages = {A9},
          doi = {10.1051/0004-6361/202244427},
archivePrefix = {arXiv},
       eprint = {2209.14495},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2022A&A...668A...9H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{URDAHL1991425,
title = {An experimental determination of the heat of formation of C2 and the CH bond dissociation energy in C2H},
journal = {Chemical Physics Letters},
volume = {178},
number = {4},
pages = {425-428},
year = {1991},
issn = {0009-2614},
doi = {https://doi.org/10.1016/0009-2614(91)90276-F},
url = {https://www.sciencedirect.com/science/article/pii/000926149190276F},
author = {Randall S. Urdahl and Yihan Bao and William M. Jackson},
abstract = {The rotational cutoff levels of C2(B′1Σ+g, ν″ = 1,2), produced in the multiphoton dissociation of jet-cooled acetylene at 193 nm, have been measured using laser-induced fluorescence. This data is used to calculate the values ΔHf,0(C2) = 194.8 ± 0.5 kcal/mol and D0(CCH) = 112.0 ± 0.8 kcal/mol, in excellent agreement with the latest theoretical calculations.}
}

@article{10.1093/mnras/138.2.143,
    author = {Lambert, D. L.},
    title = "{The Abundances of the Elements in the Solar Photosphere—I: Carbon, Nitrogen and Oxygen}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {138},
    number = {2},
    pages = {143-179},
    year = {1968},
    month = {01},
    abstract = "{ This paper discusses the determination of the abundances of carbon, nitrogen and oxygen in the solar atmosphere from an analysis of atomic and molecular spectra. A detailed discussion of the neutral atomic spectra is presented. Five molecular bands are considered: C 2 Swan Band, CN red and violet systems, CO first overtone bands, and the CH ( A2 Δ− X2 Π) band. With the exception of the CH band, the analysis of the molecular bands yields abundances which are in good accord with the results from the neutral atomic spectra. The following abundances are derived:  log AC = 8.55, log AN = 7.93 and log AO = 8.77 on the standard scale log NH = 12.00. }",
    issn = {0035-8711},
    doi = {10.1093/mnras/138.2.143},
    url = {https://doi.org/10.1093/mnras/138.2.143},
    eprint = {https://academic.oup.com/mnras/article-pdf/138/2/143/8078727/mnras138-0143.pdf},
}



@ARTICLE{2021A&A...656A.113A,
       author = {{Amarsi}, A.~M. and {Grevesse}, N. and {Asplund}, M. and {Collet}, R.},
        title = "{The solar carbon, nitrogen, and oxygen abundances from a 3D LTE analysis of molecular lines}",
      journal = {\aap},
     keywords = {radiative transfer, line: formation, Sun: abundances, Sun: photosphere, Sun: atmosphere, Astrophysics - Solar and Stellar Astrophysics},
         year = 2021,
        month = dec,
       volume = {656},
          eid = {A113},
        pages = {A113},
          doi = {10.1051/0004-6361/202141384},
archivePrefix = {arXiv},
       eprint = {2109.04752},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021A&A...656A.113A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@Inbook{Huber1979,
author="Huber, K. P.
and Herzberg, G.",
title="Constants of diatomic molecules",
bookTitle="Molecular Spectra and Molecular Structure: IV. Constants of Diatomic Molecules",
year="1979",
publisher="Springer US",
address="Boston, MA",
pages="8--689",
isbn="978-1-4757-0961-2",
doi="10.1007/978-1-4757-0961-2_2",
url="https://doi.org/10.1007/978-1-4757-0961-2_2"
}

@ARTICLE{2011ApJ...737L...7S,
       author = {{Sumangala Rao}, S. and {Pandey}, Gajendra and {Lambert}, David L. and {Giridhar}, Sunetra},
        title = "{Is the Post-AGB Star SAO 40039 Mildly Hydrogen-Deficient?}",
      journal = {\apjl},
     keywords = {stars: abundances, stars: atmospheres, stars: evolution, stars: fundamental parameters, Astrophysics - Solar and Stellar Astrophysics},
         year = 2011,
        month = aug,
       volume = {737},
       number = {1},
          eid = {L7},
        pages = {L7},
          doi = {10.1088/2041-8205/737/1/L7},
archivePrefix = {arXiv},
       eprint = {1107.1316},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...737L...7S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1998assp.book.....W,
       author = {{Wallace}, L. and {Hinkle}, K. and {Livingston}, W.},
        title = "{An atlas of the spectrum of the solar photosphere from 13,500 to 28,000 cm-1 (3570 to 7405 A)}",
         year = 1998,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998assp.book.....W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2019M&PS...54.1092B,
       author = {{Burnett}, D.~S. and {Jurewicz}, A.~J.~G. and {Woolum}, D.~S.},
        title = "{The future of Genesis science}",
      journal = {\maps},
     keywords = {Earth Science},
         year = 2019,
        month = may,
       volume = {54},
       number = {5},
        pages = {1092-1114},
          doi = {10.1111/maps.13266},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019M&PS...54.1092B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1995A&A...296..217B,
       author = {{Blackwell}, D.~E. and {Lynas-Gray}, A.~E. and {Smith}, G.},
        title = "{On the determination of the solar iron abundance using Fe I lines.}",
      journal = {\aap},
     keywords = {SUN: ABUNDANCES, ATOMIC DATA},
         year = 1995,
        month = apr,
       volume = {296},
        pages = {217},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1995A&A...296..217B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1991A&A...249..545H,
       author = {{Holweger}, H. and {Bard}, A. and {Kock}, M. and {Kock}, A.},
        title = "{A redetermination of the solar iron abundance based on new Fe I oscillator strengths}",
      journal = {\aap},
     keywords = {Abundance, Iron, Metallicity, Oscillator Strengths, Solar Atmosphere, Chondrites, Metal Ions, Photosphere, Radiative Lifetime, Solar Spectra, Transition Probabilities, Solar Physics},
         year = 1991,
        month = sep,
       volume = {249},
       number = {2},
        pages = {545-549},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991A&A...249..545H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1999A&A...347..348G,
       author = {{Grevesse}, N. and {Sauval}, A.~J.},
        title = "{The solar abundance of iron and the photospheric model}",
      journal = {\aap},
     keywords = {ATOMIC DATA, SUN: ABUNDANCES, SUN: PHOTOSPHERE},
         year = 1999,
        month = jul,
       volume = {347},
        pages = {348-354},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1999A&A...347..348G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1978MNRAS.182..249L,
       author = {{Lambert}, D.~L.},
        title = "{The abundances of the elements in the solar photosphere - VIII. Revised abundances of carbon, nitrogen and oxygen.}",
      journal = {\mnras},
     keywords = {Abundance, Electron Transitions, Gas Composition, Photosphere, Solar Atmosphere, Solar Spectra, Atmospheric Composition, Carbon, Limb Darkening, Line Spectra, Nitrogen, Oxygen, Solar Granulation, Solar Physics, Element Abundances:Solar Photosphere},
         year = 1978,
        month = jan,
       volume = {182},
        pages = {249-272},
          doi = {10.1093/mnras/182.2.249},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1978MNRAS.182..249L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1978MNRAS.183...79L,
       author = {{Lambert}, D.~L. and {Luck}, R.~E.},
        title = "{The abundances of the elements in the solar in the solar photosphere - IX: Na top Ca.}",
      journal = {\mnras},
     keywords = {Abundance, Chemical Elements, Electron Transitions, Photosphere, Radiative Lifetime, Solar Atmosphere, Atmospheric Models, Atmospheric Turbulence, Carbonaceous Chondrites, Isotropic Turbulence, Solar Physics, Element Abundances:Solar Photosphere},
         year = 1978,
        month = apr,
       volume = {183},
        pages = {79-100},
          doi = {10.1093/mnras/183.2.79},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1978MNRAS.183...79L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005MNRAS.361.1187M,
       author = {{Monteiro}, M{\'a}rio J.~P.~F.~G. and {Thompson}, Michael J.},
        title = "{Seismic analysis of the second ionization region of helium in the Sun - I. Sensitivity study and methodology}",
      journal = {\mnras},
     keywords = {equation of state, Sun: abundances, Sun: helioseismology, Sun: interior, Sun: oscillations, stars: abundances, Astrophysics},
         year = 2005,
        month = aug,
       volume = {361},
       number = {4},
        pages = {1187-1196},
          doi = {10.1111/j.1365-2966.2005.09246.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0506286},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005MNRAS.361.1187M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2007MNRAS.375..861H,
       author = {{Houdek}, G. and {Gough}, D.~O.},
        title = "{An asteroseismic signature of helium ionization}",
      journal = {\mnras},
     keywords = {Sun: abundances, Sun: oscillations, stars: abundances, stars: interiors, stars: oscillations, Astrophysics},
         year = 2007,
        month = mar,
       volume = {375},
       number = {3},
        pages = {861-880},
          doi = {10.1111/j.1365-2966.2006.11325.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0612030},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007MNRAS.375..861H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
